Deep-seeded Clustering for Emotion Recognition from Wearable Physiological Sensors

According to the circumplex model of affect, an emotional response could characterized by a level of pleasure (valence) and intensity (arousal). As it reflects on the autonomic nervous system (ANS) activity, modern wearable wristbands can record non-invasively and during our everyday lives peripheral end-points of this response. While emotion recognition from physiological signals is usually achieved using supervised machine learning algorithms that require ground truth labels for training, collecting it is cumbersome and particularly unfeasible in naturalistic settings, and extracting meaningful insights from these signals requires domain knowledge and might be prone to bias. Here, we propose and test a deep-seeded clustering algorithm that automatically extracts and classifies features from those physiological signals with minimal supervision - combining an autoencoder (AE) for unsupervised feature representation and c-means clustering for fine-grained classification. We also show that the model obtains good performance results across three different datasets frequently used in affective computing studies (accuracies of 80.7% on WESAD, 64.2% on Stress-Predict and 61.0% on CEAP360-VR).

==> old/oldtext.tex <==

\section{PREV VERSION}
The American Institute of Stress defines stress as a “condition or feeling experienced when a person perceives that demands exceed the personal and social resources the individual is able to mobilise” \cite{AIS}. Stress is a fundamental cerebral phenomenon that enables the expenditure of a big quantity of energy to solve a given problem \cite{garces2019emotional}. This energy is both cognitive and physical. On the one hand, the highest is the stress level, the highest the being considers the problem as a priority. On the other hand, the body consumes a high quantity of energy to prepare and carry out an intense physical reaction: the cardiovascular system accelerates, the sudoriparous glands secrete sweat, vasoconstriction decrease the skin temperature, muscles tighten, etc...\cite{giannakakis2019review}. Thereby, stress is both a psychological and physical response.\par
Nonetheless, stress is not necessarily unpleasant. Writing a report can be stressful but enjoyable, for example. Positive stress is called "eustress" and negative stress is called "distress". In general, high level of stress is perceived as a negative feeling but when the being feels close to solve a difficult problem the stress is perceived as positive. As detailed in \cite{hancock2008performance}, facing a complex problem under light stress tends to increase performance contrary to high stress. Actually, high stress paralyses the being’s reasoning, or learning process, while favouring automatic responses \cite{yerkes1908relation}, \cite{garces2019emotional}. Under overwhelming stress, the being reacts with simple innate responses like Canon’s "fight or flight" responses \cite{cannon1939wisdom}.\par
Prolonged stress periods expose humans to sever diseases such as depression, obesity and stroke \cite{kasl1984stress}. Monitoring stress may help to identify and neutralise excessive or useless stressors.\par
% literature review
Stress can be measured by simply asking people to assess their stress level. However, stress level is a continuous process and no one can assess one’s stress level in continuous time. Worse still, people can hardly assess their stress level when they are preoccupied. They can assess it after facing the problem. Unfortunately, agents’ remembered emotions tend to be biased from what they actually felt \cite{lima2018dynamic}, \cite{redelmeier1996patients}, \cite{fredrickson1993duration}. Finally, measuring stress through questionnaires implicitly assumes that respondent are able to assess their emotions and that they answer honestly. These two assumptions should be questioned in various cases \cite{smith1997impact}, \cite{caputo2017social}.\par
Fortunately, stress is also a physiological phenomenon. Thus, measuring the end-points of the physiological stress response reveals the individual’s stress level. The sweat secretion increases the skin’s electric conductivity, electrodermal activity (EDA). The cardiovascular system acceleration increases the veins blood flow, or blood volume pulse (BVP). The vasoconstriction decreases the skin temperature (ST) by reducing the amount of warm blood from the heart in the superficial tissues.\par
Numerous studies has tried to detect stress from these three bio-signals. Online methods often analyse the signals’ frequency bands. When a particular band is intense, the individual is considered as stressed \cite{rani2002online}, \cite{kyriakou2019spatial}. These methods are fast but lack reliability.\par
Supervised learning models, like neural networks, identify stress with satisfying accuracy \cite{gedam2020automatic}. Unfortunately, supervised learning models, especially neural networks, are in general barely generalisable. Worse still, collecting labels requires to know all stressors in the individual’s environment, at least most of them. Anyhow, defining ground truth is questionable \cite{schmidt2018introducing}. Recently, unsupervised clustering has emerged as a promising alternative to the lack of labels \cite{zhao2018emotionsense}, \cite{huysmans2018unsupervised}, \cite{maaoui2018unsupervised}, \cite{vildjiounaite2017unsupervised}, \cite{wu2020unsupervised}. First, signals are sliced and features are extracted from each slice. Then, the features are classified. This approach requires signal theory and physiology expertise. Moreover, no feature, nor list of features, may completely reflect the useful information held in a signal slice. Aqajari \cite{aqajari2021pyeda} used an auto-encoder to automatically extract features. Unfortunately, he classified these features with supervised learning.\par
In this article, we leverage the power of deep-clustering \cite{yang2017towards}. This algorithm revealed to be efficient for unsupervised computer vision \cite{caron2018deep}, \cite{yang2016joint}. Jointly, a sequence-to-sequence auto-encoder extracts features from the EDA, BVP and ST bio-signals and clusters these features. We implement the algorithm proposed by Yang \textit{et al.} \cite{yang2017towards}. Tests on the WESAD data set \cite{schmidt2018introducing} reveal that our method outperforms unsupervised, and supervised learning algorithms for detecting stress.\par
In Section~\ref{section:related_work}, we review stress detection methods.
In Section~\ref{section:methodology}, we detail the pre-processing of the EDA, BVP and ST signals. In addition, we explain the functioning of a sequence-to-sequence auto-encoder and a deep-cluster algorithm. In Section~\ref{section:experimetal_evaluation}, we evaluate the performance of our method. In Section~\ref{section:conclusion}, we conclude with general remarks.\par

